New kids on the block: an analysis of modern blockchains

Half a decade after Bitcoin became the first widely used cryptocurrency, blockchains are receiving considerable interest from industry and the research community. Modern blockchains feature services such as name registration and smart contracts. Some employ new forms of consensus, such as proof-of-stake instead of proof-of-work. However, these blockchains are so far relatively poorly investigated, despite the fact that they move considerable assets. In this paper, we explore three representative, modern blockchains---Ethereum, Namecoin, and Peercoin. Our focus is on the features that set them apart from the pure currency use case of Bitcoin. We investigate the blockchains' activity in terms of transactions and usage patterns, identifying some curiosities in the process. For Ethereum, we are mostly interested in the smart contract functionality it offers. We also carry out a brief analysis of issues that are introduced by negligent design of smart contracts. In the case of Namecoin, our focus is how the name registration is used and has developed over time. For Peercoin, we are interested in the use of proof-of-stake, as this consensus algorithm is poorly understood yet used to move considerable value. Finally, we relate the above to the fundamental characteristics of the underlying peer-to-peer networks. We present a crawler for Ethereum and give statistics on the network size. For Peercoin and Namecoin, we identify the relatively small size of the networks and the weak bootstrapping process.

==> bitcoin.tex <==
\section{Bitcoin: the grandfather}
\label{sec:bitcoin}

\subsection{Network}


==> contract_analysis_levdist_table.tex <==
\begin{table}[]
\centering
\caption{Contract and Levenshtein Distance}
\label{tab:contract-levenshtein}
\begin{tabular}{@{}lllll@{}}
\toprule
\multicolumn{2}{l}{\multirow{2}{*}{Tutorial Contract}} & \multicolumn{3}{c}{Levenshtein Distance ($\delta$)}                                \\ 
\multicolumn{2}{l}{}                                   & $\delta=0$ & $0<\delta \leq 100$  & $100 < \delta \leq 1000$ \\ \midrule
\multirow{2}{*}{Ballot\footnote{http://solidity.readthedocs.io/en/latest/solidity-by-example.html\#voting}}               & optim          & 7         & 1                                & 3                                   \\
                                      & non-optim      & 0         & 0                                & 0                                   \\ \midrule
\multirow{2}{*}{Blind Auction\footnote{http://solidity.readthedocs.io/en/latest/solidity-by-example.html}}                & optim          & 0         & 0                                & 0                                   \\
                                      & non-optim      & 0         & 0                                & 0                                   \\ \midrule
\multirow{2}{*}{Coin\footnote{https://ethereum.gitbooks.io/frontier-guide/content/contract\_coin.html}}                 & optim          & 94        & 1                                & 8815                                \\
                                      & non-optim      & 18        & 93                               & 9311                                \\ \midrule
\multirow{2}{*}{Crowdsale\footnote{https://www.ethereum.org/crowdsale}}            & optim          & 4         & 0                                & 29                                  \\
                                      & non-optim      & 1         & 0                                & 15                                  \\ \midrule
\multirow{2}{*}{Greeter\footnote{https://www.ethereum.org/greeter}}              & optim          & 127       & 47                               & 9183                                \\
                                      & non-optim      & 39        & 11                               & 6776                                \\ \midrule
\multirow{2}{*}{Mortal\footnote{https://www.ethereum.org/greeter}}               & optim          & 7         & 48                               & 8669                                \\
                                      & non-optim      & 11        & 7                                & 8827                                \\ \midrule
\multirow{2}{*}{Safe Remote Purchase\footnote{http://solidity.readthedocs.io/en/latest/solidity-by-example.html}}             & optim          & 0         & 0                                & 5137                                \\
                                      & non-optim      & 0         & 0                                & 0                                   \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Simple\\ Auction\footnote{http://solidity.readthedocs.io/en/latest/solidity-by-example.html}\end{tabular}} & optim     & 1     & 0     & 6761                                \\
                                      & non-optim      & 0         & 0                                & 0                                   \\ \midrule
\multirow{2}{*}{Token\footnote{https://www.ethereum.org/token}}                & optim          & 0         & 2728                             & 5965                                \\
                                      & non-optim      & 0         & 1                                & 8906                                \\ \midrule
\end{tabular}
\end{table}

==> ethereum_arbitrary_data.tex <==
\subsection{Poisoning of Ethereum}
In Ethereum, arbitrary data can be included in any transactions and contract creations. This potentially poses a threat of poisoning the blockchain. We analyse the Ethereum public blockchain to identify arbitrary data that are included in any transactions. 

We look at the input data of every transactions in Ethereum and extract the first 6 characters, including ``0x''. These six characters are then matched to our database of signatures of commonly used file formats. For every match, we convert the input data from hexadecimal string into its binary form using ``xxd -p -r''. Using the first 6 characters can result in high false positive and might not provide the best coverage. For instance, we will miss a file if it is embedded in a contract creation deployment script.

We scan for 75 different file formats, including exe, doc, jpg, png, pdf, gzip, tar.gz, and mp3. We found 2 pngs, 1 jpeg, 1 mp3 and 1 tar.gz.
One of the png is a text of ``gartenzwerg'' while the other is a corrupted png of bitcoin logo. The jpeg that we found is very disturbing and would be classified as not safe for work. We extract the tar.gz file and saw a letter.

\todo{include txHash for each of these perhaps?}

==> ethereum_peer_crawler.tex <==



==> network.tex <==
\section{Investigating the blockchain networks}






\subsection{Network statistics}

